Uncovering Urban Mobility and City Dynamics from Large-Scale Taxi Origin-Destination (O-D) Trips: Case Study in Washington DC Area

We perform a systematic analysis on the large-scale taxi trip data to uncover urban mobility and city dynamics in multimodal urban transportation environments. As a case study, we use the taxi origin-destination trip data and some additional data sources in Washington DC area. We first study basic characteristics of taxi trips, then focus on five important aspects. Three of them concern urban mobility, which are respectively mobility and cost including effect of traffic congestion, trip safety, and multimodal connectivity; the other two pertain to city dynamics, which are respectively transportation resilience and the relation between trip patterns and land use. For these aspects, we use appropriate statistical methods and geographic techniques to mine patterns and characteristics from taxi trip data for better understanding qualitative and quantitative impacts of the inputs from key stakeholders on available measures of effectiveness on urban mobility and city dynamics, where key stakeholders include road users, system operators, and city. Finally, we briefly summarize our findings and discuss some critical roles and implications of the uncovered patterns and characteristics from the relation between taxi system and key stakeholders. The results can support road users by providing evidence-based information of trip cost, mobility, safety, multimodal connectivity and transportation resilience, can assist taxi drivers and operators to deliver transportation services in a higher quality of mobility, safety and operational efficiency, and can also help city planners and policy makers to transform multimodal transportation and to manage urban resources in a more effective and better way.

==> ideas.tex <==
\section{Raw Ideas}

\subsection{Macroscopic Structure}

\cite{louail2015uncovering} \cite{hamedmoghadam2017complex}  I, C, D, R 

\subsection{Studying Zones}

\subsubsection{r-digit zones} 

\subsubsection{census tracts} 

\subsubsection{Traffic analysis Zone (TAZ)}

\cite{yang2018analysis} 

\subsubsection{Voronoi tessellation}

Bikeshare Stations: \cite{mckenzie2018docked}(DC)


Metro Stations: 

\subsubsection{Zone Mapping}

- Within Approximation: Large Zones to tiny Zones (e.g., r-3 zones)

- Intersection of Zones: Large Zones to Large Zones

\subsection{Regression models}

\cite{yang2018analysis} Ordinary Least Square (OLS) regression models to relate taxi demand with land use characteristics (retail, office, industry and other; entropy variable), and transit supplies (accessibility to other modes).

different types of employment on the demand for for-hire rides

$R^2$

\subsection{comparative Studies}

- Check the impact of accidents on traffic congestion (temporal and spatial)

- shareability: proportion of taxi trips that are shareable

- relation with metro/transit/bike

household travel survey data: rely on a costly and time consuming process

NYC: The land use falls under six categories: Residential (R), Commercial (C), Industrial & Manufacturing (I), Transportation (T), Public Institutions (P), and Open Space & Outdoor Recreation (O).

\subsection{Mode characteristics}

Transport modes in urban transportation systems provide passenger services with different levels of convenience, flexibility, and economic benefits. The travel demands generated from these modes are both shaped by factors such as population size, land use patterns, and other socio-demographic characteristics. However, there exist different socio-economic processes
that govern individual and collective choices over one mode to the other.

\subsubsection{taxi}

Unlike public transit, deployment of taxi service does not require
high population density. It can be taken from anywhere, not constrained by a limited number of pick-up locations, although the service
may be more accessible in some areas. In the areas where no public
transit is provided, taxi complements its service; while it also competes
with public transit as an alternative transport means with high flexibility in time and at a higher cost.

\subsubsection{transit}

The public transportation system is only considered by city government when
population density reaches a certain level. Accessibility to transit service
is higher around bus stops or metro stations than other places. It
means intra-urban connectivity by public transit is enhanced at areas
around bus stops or metro stations but not uniformly along bus/metro route.

\subsubsection{mobility patterns}

Urban travel patterns are the outcome of the complex interactions between land use configuration and individual characteristics. The land use system governs spatial distribution of opportunities (in commercial, industrial areas) and the demand for these opportunities (in residential areas). The classical urban transport model as-
sumes the trip amount between different zones is proportional to the
number of households at the origin and the number of opportunities at
the destination. However, when zooming into local neighborhood, the
share disparity of different transport modes is more sensitive to in-
dividual characteristics such as income, education and vehicle owner-
ship. This share disparity is captured in mode choice model which is
used to forecast individuals' travel behaviors based on microeconomic theory.

Human mobility datasets generated by public transportation and
taxi can be used to reveal urban travel patterns. Mining the variances of
the travel patterns will provide hints related to the local land use, socio-
demographics, and the city structure. For example, a temporal profile of
outgoing and incoming trips can be used to infer land use. The mode share disparity may suggest differences of socio-
demographics in different areas. Also, the flow of people and goods
connects urban spaces which may have implications for spatial inter-
actions in different regions. These spatial interactions reflect economic
activities and reveal the underlying urban structures.

\subsubsubsection{spatial distribution of travel demand}

The Spearman's rank correlations of travel demand: That means public transit and taxi usages are highly comparable in many areas and this is possibly driven by factors such as population distribution and spatial configuration of land use. There are some discrepancies of travel demand in particular regions.

\subsubsubsection{statistical properties of collective travel behavior}

travel distance of trips and its spatial distribution in the city (e.g., distance decay effect)

Travel distance is another important metric that reflects the spatial structure of human movements.

- Median travel distance for both incoming and outgoing trips at the subzone level: compare the geographic variations of travel distance (degree of spatial heterogeneity), smooth variation over space; The trips that started in the central part of Singapore are relatively short as compared to the ones that originated from the outer subzones

- probability of trips at different distance values: distance decay effect

\subsubsubsection{urban structures}

spatial interactions of urban spaces revealed from trip OD based spatial network.

- community detection: a technique that has been widely used to uncover hidden structures in networks to assess whether the two transport layers produce similar or different spatial interaction patterns.


\subsubsection{Analysis methods}

\subsubsubsection{rank-size distribution}

\subsubsubsection{{log odds ratio}

comparative: spatial, complex network

Different spatial granularities: map trip origins/destinations onto subzones

\subsubsection{Complex Networks}

\input{../stats/complexnetwork}

\subsubsection{Analysis Miscs}

Weekday/Weekend (temporal): mobility patterns might be different on weekdays and weekends


\subsection{Extra Info}

Travel time is another important indicator to analyze the human mobility. From the aspects of geography, travel distance discovers the spatial information. While travel time reflects the travel accessibility and traffic condition in urban road network. 

\cite{wang2017new} According to the 2010/2011 RHTS data, the taxi has a mode share of about 1.01\% in the 28 counties of the NY-NJ-CT metropolitan area.

\cite{koster2011travel} Travellers minimize their expected access costs to the airport,
EðCðHÞÞ by deciding on the optimal safety margin H when departing from home. They
take into account this safety margin because travel times may exceed free-flow travel time.

\cite{wang2015comparative} the displacement of each occupied trip, the duration of each occupied trip, and the time interval between successive occupied trips by the same taxi (interevent time)

\cite{tang2016two} Huff model is used to describe the attractiveness of a pick-up area, considering the historical number of pick-up passengers and distance between drop-off and pick-up areas as
explanatory variables.

\cite{castro2013taxi} three main categories: social dynamics, traffic dynamics and operational dynamics. Social dynamics refers
to the study of the collective behaviour of a city’s population, based on their observed movements; Traffic
dynamics studies the resulting flow of the movement through the road network; Operational dynamics refers
to the study and analysis of taxi driver’s modus operandi. 

\cite{qin2017mining} Supply-demand ratio, search distance, fare and delivery speed are the four significant factors affecting incomes,
while search intensity is insignificant. The insignificance of search intensity indicates that searching passengers
through routes in a high likelihood of pickups is not a rule of thumb to increase incomes.

\cite{liu2012urban} land use

%./dc_taxidata_1Y_r2_38.89_-77.01_hod_Week.eps Union Station

\cite{qi2011measuring} get-on/off amount in a region can depict the social activity dynamics in that area, i.e. the temporal variation of get-on/off amount can characterize the social function of a region.

free-floating vehicles

Monitoring, predicting and understanding traffic conditions in a city is an important problem for city planning and environmental monitoring.

Airport Accessibility: Taxi data 

When the drivers send a passenger to destination, they will quickly move to the possible pick-up locations based on their experience. 

The reason can be explained from following two aspects: (1) the size of urban area and structure of network limit
the travel space of taxi trips. Very long trips (d > 15 km, t > 50 min) take small part of all the trips. (2) the economic
condition is another factor. Taxi fare will increase as travel distance and time accumulate. Too short or too long trips are
not economical. Generally, walk and bicycle are favorite transportation ways for short trips, and most people will choose
subway and bus for long trips. 

\cite{correa2017exploring} A high correlation between taxi and Uber pick-ups can be observed.

\cite{correa2017exploring} Neighborhoods with lower transit access time (TAT), higher length of roadways, lower
vehicle ownership, higher income and more job opportunities are associated with higher taxi/Uber demands.

\subsubsection{Main Pictures}

Fig (Basic Descriptions): Year, season, Week

Fig (qgis): Spatial Description of Pickup and Dropoff

Fig (Travel Description): Travel Time, milage, Speed, Cost

Fig (temporal): (Speed,Cost) during different TOD 

Fig (temporal): (Speed,Cost) in different Miles 

Fig (Spatial): Cases (Region, Week, LBSN) (Airport, Union Station, Food, Career, Recreation) 

Table: 4SQ Data on (Airport, Union Station, Food, Career, Recreation) 

Fig (Special diruptions): Metro Shutdown (Travel Time, milage, Speed, Cost)

Fig (Connection to other modes): (metro and bikeshare)

\subsubsection{Time distribution}
%runKolmogorovSmirnovTester.sh -i1 dc_taxidata_1Y_col_TripSpeed_Weekday_3+3.csv -i2 dc_taxidata_1Y_col_TripSpeed_Weekday_15+3.csv

[smos.ext.data.analysis.KolmogorovSmirnovTester]
[2017-06-13 10:25:58 | INFO] val1=244520
[2017-06-13 10:50:43 | INFO] val2=2410056
[2017-06-13 10:50:43 | INFO] p=0.0

\subsubsection{Transportation Hubs}

the number of trips originating at the train stations remains roughly constant from Monday through Thursday, and starts to decrease on Friday, hitting a low on Saturday.

\subsection{Disruptions}


\subsubsection{Metro Shutdown 1601 Blizzard}
January 2016 United States blizzard

"2016-01-21","46227"
"2016-01-22","21682"
"2016-01-23","282"
"2016-01-24","3672"
"2016-01-25","16690"
"2016-01-26","22791"
"2016-01-27","35498"
"2016-01-28","43270"

BPCount
"2016-01-23","90"
"2016-01-24","155"
"2016-01-25","418"
"2016-01-26","877"

CaBi:
"2016-01-21","4228"
"2016-01-22","2985"
"2016-01-23","0"
"2016-01-24","0"
"2016-01-25","0"
"2016-01-26","0"
"2016-01-27","528"
"2016-01-28","2022"

\subsubsection{Metro Shutdown 160316}

Increased from 48665.5 to 60153: 23.6\%
Metro 2016 Ridership: 639,101

Hour	Mon	Tue	Wed	Thu	Fri	Sat	Sun		Weekdays	Weekday	Weekend		Total	Avg	2016-03-16	delta
0	614.3333333	620.3333333	695	797.6666667	1077.666667	2127.666667	2638.333333		3805	761.0	2383		8571	1224.4	744	0.9776609724
1	376.6666667	355.3333333	416.3333333	448	709.6666667	1879.333333	2497		2306	461.2	2188.166667		6682.333333	954.6	418	0.9063313096
2	259.3333333	192	241.3333333	271.6666667	404	1684	1655		1368.333333	273.7	1669.5		4707.333333	672.5	234	0.8550548112
3	118.6666667	105.6666667	125.6666667	130.3333333	178.3333333	860	1278.333333		658.6666667	131.7	1069.166667		2797	399.6	119	0.903340081
4	203	177.3333333	240.6666667	263.3333333	248.6666667	374	659.6666667		1133	226.6	516.8333333		2166.666667	309.5	285	1.25772286
5	359.3333333	326	454.6666667	400.6666667	355.3333333	330	400.6666667		1896	379.2	365.3333333		2626.666667	375.2	610	1.608649789
6	741	738.6666667	869.3333333	785.6666667	583.3333333	469.3333333	487.6666667		3718	743.6	478.5		4675	667.9	1281	1.722700377
7	1565.333333	1806.333333	1835.333333	1696	1116.666667	593.3333333	616.6666667		8019.666667	1603.9	605		9229.666667	1318.5	2382	1.485099131
8	2381.666667	2705.333333	2759.666667	2659.333333	1831.666667	823.6666667	914		12337.66667	2467.5	868.8333333		14075.33333	2010.8	3111	1.260773242
9	2652	3068	3017	2973.333333	2231	1139.666667	1286.333333		13941.33333	2788.3	1213		16367.33333	2338.2	3283	1.177434009
10	2532	3108.666667	2899	2912.666667	2343	1334.666667	1543.666667		13795.33333	2759.1	1439.166667		16673.66667	2382.0	3051	1.105808728
11	2765.333333	3539	3428	3297.666667	2435	1742.666667	1661.333333		15465	3093.0	1702		18869	2695.6	3703	1.197219528
12	2829	3593	3436	3415.666667	2149	1957.666667	1731.666667		15422.66667	3084.5	1844.666667		19112	2730.3	3771	1.222551223
13	2925.333333	3806	3691	3580	2213	1931.666667	1658.333333		16215.33333	3243.1	1795		19805.33333	2829.3	4015	1.238025737
14	3018	3730.666667	3667.333333	3589	2278.333333	2171	1935		16283.33333	3256.7	2053		20389.33333	2912.8	4216	1.29457523
15	3014.333333	3598.666667	3612.666667	3559.666667	2242	2487.333333	2265.333333		16027.33333	3205.5	2376.333333		20780	2968.6	4195	1.308701801
16	3012	3391.333333	3494	3283.333333	2224.666667	2386.333333	2220.666667		15405.33333	3081.1	2303.5		20012.33333	2858.9	3932	1.276181409
17	3075	3440.666667	3414	3209	2273.333333	2548.666667	2097.666667		15412	3082.4	2323.166667		20058.33333	2865.5	3909	1.268167662
18	3112	3336.333333	3409.333333	3226.666667	2386.333333	2733.666667	2071.333333		15470.66667	3094.1	2402.5		20275.66667	2896.5	3972	1.283719728
19	2717.333333	2775	3001	2903.333333	2001.333333	2611.333333	1755		13398	2679.6	2183.166667		17764.33333	2537.8	3442	1.284520078
20	2388	2632.333333	2715.666667	2782.333333	1815.666667	2177	1567.333333		12334	2466.8	1872.166667		16078.33333	2296.9	3048	1.235608886
21	2208	2500.333333	2667.333333	2671	1841.666667	2283.333333	1643		11888.33333	2377.7	1963.166667		15814.66667	2259.2	2890	1.215477359
22	1769.333333	1930	2029.666667	2316.666667	1916.333333	2507.333333	1474.666667		9962	1992.4	1991		13944	1992.0	2220	1.11423409
23	1031.666667	1188	1312	1675.666667	1857.333333	2590.666667	1091		7064.666667	1412.9	1840.833333		10746.33333	1535.2	1322	0.9356421629
SUM	45668.66667	52665	53432	52848.66667	38713.33333	41744.33333	37149.66667		243327.6667	48665.5	39447		322221.6667	46031.7	60153.0	1.236049333

- 
